Properties and Applications of Programs with Monotone and Convex Constraints

We study properties of programs with monotone and convex constraints. We extend to these formalisms concepts and results from normal logic programming. They include the notions of strong and uniform equivalence with their characterizations, tight programs and Fages Lemma, program completion and loop formulas. Our results provide an abstract account of properties of some recent extensions of logic programming with aggregates, especially the formalism of lparse programs. They imply a method to compute stable models of lparse programs by means of off-the-shelf solvers of pseudo-boolean constraints, which is often much faster than the smodels system.

==> response-to-editor <==
Dear Professor Rossi,

We are sending to you a revised version of paper 2009. We read the
reviews and took all the comments into consideration. Please, find
below a detailed account of how we revised the paper.

Reviewer 1: we corrected the typo pointed in the review (the only comment that
required attention)

Reviewer 3: we decided to keep the experimentation section in the paper. It
serves as a verification of the usefulness of our results and shows 
that our system pbmodels is effective (often faster than smodels), even 
with the present generation of PB solvers.

The majority of comments, corrections and suggestions came from Reviewer
2. In most cases, we followed the suggestions offered. Below, we cite the 
comments of Reviewer 2 and follow each with a comment (marked LLMT) on 
how we reacted.

1. some proofs skip some interesting details, while others enter into
tedious details that are probably not as interesting. Perhaps it would
be a good idea to move the proofs to the appendix (to facilitate reading 
the paper) and ensure uniformity in their development.

LLMT  The proofs are relatively short and only two approach the length
LLMT  of one page. Thus, we feel having proofs in the main part of the
LLMT  paper does not adversely affect the overall flow of reading.

2. there are some minor inconsistencies in some proofs

3. the related work section is rather unsatisfactory. First of all, 
there are some relevant papers that have not been mentioned. Second, the 
comparison with the existing results is almost non-existent. The 
framework proposed in this paper is motivated as a way to handle general 
classes of aggregates, without restriction on where they are used (e.g., 
as heads of rules). In particular, a range of semantic characterizations 
of aggregates in LP have appeared in recent years (and some are cited in 
the introduction). Nevertheless, there is no comparison between the 
semantical characterizations proposed in the literature (e.g., Pelov's 
work, Faber et al.) and the semantics captured by your approach. This is, 
n my opinion, a serious drawback.

LLMT  General comments (2) and (3) are addressed through our reaction to
LLMT  detailed comments listed below.

Detailed Comments:

I will provide some more detailed comments, following the presentation in the
paper.

INTRODUCTION:
This is the only place where related work is mentioned (apart for some
later references to Smodels and weight constraints). I would like to see
a separate section dedicated to related work, which includes more formal
comparisons. E.g., if we consider modeling aggregates as constraints, what
sort of semantics is captured?

Also:
* when citing [6,24,5,25,10] you talk about papers that deal with
   "constraints"; all these papers make use of the term "aggregates" instead.
   This difference in terminology should be explained. Also, some people
   might be a bit misled by the term "constraint" (as it is used in a
   different framework than the common use of "constraint" in "Constraint
   Logic Programming").

LLMT We included a comment on this issue in the (new) section Related work

* there are some references that are missing. Apart for some other proposals
   on semantics and/or implementation of aggregates (e.g., [1,2,3]) there is
   the very important work by Ferraris [4]. In particular, I would have
   really liked a comparison with the material in [4].

LLMT We added comments on related papers in the (new) section Related
LLMT work

PRELIMINARIES:
This section is quite well-written, though it could benefit of some more
discussion and some examples. In particular,
* provide some intuition behind some of the definitions. For example, I
   found a bit unintuitive the definition of supported model.

LLMT  We included in the paper examples to illustrate the concept of
supportedness. (page 5)

* it would be nicer to have a formal definition of T_P^{nd}

LLMT  The definition we have in the paper is precise.

* in this section and in some later ones, the notion of lparse programs is
   repeated; it would be nice to have a formal definition here of lparse
   programs (essentially the definitions in Section 8.1). I have also found
   a bit misleading talking about lparse programs here, since the constraints
   described do not allow upper bounds.

LLMT  In this place of the paper, lparse programs appear only as a 
LLMT  justification for introducing cardinality and weight constraints, and 
LLMT  for the notation we use for them. So, we decided to leave formal
LLMT  definitions of lparse programs where they currently are (section 8.1).
LLMT  However, we rephrased slightly the text to make it clearer.

* Equation (2) is identical to equation (1), perhaps you could avoid
   repeating it.

LLMT  We eliminated the redundant equation.

* The symbol 't' is used with two different meanings (length of the
   computation in page 5 and P-computation in page 6). I would recommend
   using different symbols.

LLMT  This is not the case. We consistently use the term $\alpha_t$ to
LLMT  denote the *length* of a *computation* $t$.

* since in page 7 you talk about minimal models, it would be nice to have a
   discussion of minimality properties of derived models. If I am not wrong,
   it should be possible to have programs with more than one minimal
   derivable model (even without default negation). It would be nice to see
   some examples of this.

LLMT  We added a discussion of this issue. (page 8)

* in section 2.2 there is no need of saying 'monotone-constraint' since you
   have already mentioned that implicitly the programs are assumed to have
   only monotone constraints. Indeed, results in pages 6/7 rely heavily on
   monotonicity (you should perhaps stress this fact, and maybe show examples
   of why monotonicity is important).

LLMT  We want to keep the word "monotone-constraint" in our theorems and
LLMT  definitions in Section 2.2 since it provides a clear context within 
LLMT  which our theorems hold.

* in page 8, it would help to have a brief lemma stating that models of
   P^M are models of P

LLMT  This lemma is very easy to show and we decided not to include this
LLMT  result. However, we reformulated the proof slightly.

* section 2.2 really needs at least one example of a program and one or more
   stable models.

LLMT  We included a simple example (page 11)

* since we are looking at constraint atoms as a generalization of
   traditional LP, it would be nice to have a discussion that relates the
   two. I.e., if we take a standard LP and we replace each atom b with its
   ({b}, {{b}}) constraint, we are guaranteed a correspondence with
   traditional stable models.

LLMT  This result is proved in \cite{nmt04}. We will add the reference 
LLMT  in the paper.

STRONG AND UNIFORM EQUIVALENCE:
This section is quite solid. Just some minor suggestions:
* provide a little bit of motivation behind the two notions of equivalence

LLMT  We included an additional paragraph at the very beginning of Section 3
LLMT  to provide some intuition.

* in Definition 3, probably the 'M be its model' should be changed to
   'M be a model'

LLMT  We made the correction

* Proposition 7: the wording ("is the least M-maximal model") suggests
   that there is only one least M-maximal model. Is it the case? Somehow
   that is not clear to me, and it should be discussed. As a matter of
   fact, the example in page 9 seems to suggest otherwise.

LLMT  In fact this is precisely what we mean. Can(P,M) *is* the least
LLMT  $M$-maximal model, that is, it is included in every other
LLMT  $M$-maximal model. Our proof shows this. Being least, Can(P,M) is 
LLMT  the unique minimal $M$-maximal model

* in the proof of proposition 7, I would recommend the following changes:
   - the last paragraph should be the first thing to prove

LLMT  We changed the structure of the proof

   - when you perform the induction, clearly state what are you proving by
     induction (i.e., X_{\alpha}\subseteq N')

LLMT  We modified the proof accordingly.

* please provide some intuition and examples of SE models

LLMT We added some discussion and a simple example. (page 14)

* in page 11, again, there is a wording that is confusing "M is the least
   M-maximal model of P^M"; is it unique? If so, please state it explicitly
   (and prove it).

LLMT  We addressed this point above.

* please provide some intuition and examples of UE models and Uniform
   equivalence; also, please relate these concepts more clearly to the
   corresponding concepts in standard LP

LLMT  We included an example (page 16). We also state on page 12 that
LLMT  under the natural representation of normal programs as constraint 
LLMT programs (discussed, for instance in [MNT04]) our concepts and 
LLMT results related to strong and uniform equivalence reduce to those
LLMT in standard LP.

* proof of lemma 5 is probably more detailed than it should be (it is a
   fairly easy proof).

LLMT  Indeed, the proof is easy. As it is also quite short proof, we decided
LLMT  to keep it as it is.

LOGIC PL^{mc} and COMPLETION
This is a nice section. The only suggestion would be to (again) include some
explanatory examples. Also, perhaps the section could close with some
considerations that extends Theorem 4 to the situation covered by Theorem 3.

LLMT  We included the result suggested by the reviewer. (page 23)

LOOPS and LOOP FORMULAS
* In page 18, I would recommend to make explicit (in words) the fact that by
   writing "A \in bd(r)" you focus on the "positive" part of the body of r

LLMT  We modified the text accordingly. (page 23)

* I would rewrite the sentence "Thus, maximal loops are ..." as
   "Thus, (maximal) loops are...."

LLMT  This is not correct. Loops are sub-graphs that are strongly 
LLMT  connected. Only maximal loops are strongly connected components.

* The definition of A_{|L} seems a bit odd. This is still supposed to be
   a constraint but I do not see a domain in this formula (X). Also, the
   formula contains a '}' that was never opened. It would help here to provide
   an intuitive description of what you are defining (keep only the solutions
   of the constraint that are "away" from L?). Again some examples would also
   help in the understanding.

LLMT  This is a typo. We fixed it.

* The proof of Theorem 5 is rather confusing. For example, the first part
   of the second paragraph (the case M\cap L =\emptyset) is unclear. What is
   'r' here?

LLMT  This is a typo. We want to say "If $M\cap L=\emptyset$ then 
LLMT  $M\models LP(L)$." We made the change.

   In the third paragraph, shouldn't the P(X_{n-1}) be P^M(X_{n-1})?

LLMT  You are right. We fixed it.

* Section 6 needs some closing discussion about the relevance of the results

LLMT We added some comments on this issue. (page 26)

PROGRAMS WITH CONVEX CONSTRAINTS
This section seems to have been written a bit in a rush, and should be
improved.

* I am a bit puzzled by the discussion at the beginning of page 21; the
   transformation mc(.) is defined for constraint atoms; thus, in the
   construction of r', when you write {mc(A): A\in bd(r)} I am assuming
   that A is a constraint atom. On the other hand, the definition of convex
   program  (page 20) is built on equation 1, which contains default negation.
   Are default negations omitted in constructing r'? Or is mc extended to deal
   also with not A literals?

LLMT  We changed the definition of cc programs so that "not" does not
LLMT  appear in the rules. (page 26)

* instead of using running text, to be consistent with the rest of the paper,
   the semantics of convex constraint program should be formalized as a
   definition, along with formal definitions for its semantics. Similarly, the
   part where you define cc should be formalized instead of writing it as it
   is now.

LLMT  We made the change as requested. (page 27)

* please provide a formal proof of Theorem 7

LLMT  Checking that Comp(mc(P)) and Comp(P) is tedious but
LLMT  straightforward. Thus, we decided not to expand our proof sketch to 
LLMT  a full argument.

APPLICATIONS
* page 24: please provide a formal argument for the convexity of (X,C)

LLMT  We added an argument to the section to show weight atoms are indeed
       convex constraints. (page 31)

* the discussion in the remark of page 24 is really vague (e.g., removal of
   negative weights). Please formalize.

LLMT  We added the reference to paper SNS02 and MNT06. That paper has a
       detail description of how negative weights are removed. We also
       rephrased the Remark to clarify this issue. (page 31)

* page 25: please make use of indices in the \bigsum formulae

LLMT  We modified the text accordingly

* the term 'PB constraint' is used without being defined

LLMT  It is a shorthand for "pseudo-boolean constraint". We made it
LLMT  explicit in the definition of a pseudo-boolean constraint. (page 32)

* in page 25, please don't use \rightarrow to denote the transformation of F
   (it is too similar to an implication)

LLMT  That is a valid comment. We changed the notation.

* in page 27 there is a reference to a Corollary 9 that I could not locate
   (Theorem 9 perhaps?)

LLMT  Indeed, it should be Theorem 9. We made the correction

